Homotopy theories of $(\infty, \infty)$-categories as universal fixed points with respect to enrichment

We show that both the $\infty$-category of $(\infty, \infty)$-categories with inductively defined equivalences, and with coinductively defined equivalences, satisfy universal properties with respect to weak enrichment in the sense of Gepner and Haugseng. In particular, we prove that $(\infty, \infty)$-categories with coinductive equivalences form a terminal object in the $\infty$-category of fixed points for enrichment, and that $(\infty, \infty)$-categories with inductive equivalences form an initial object in the subcategory of locally presentable fixed points. To do so, we develop an analogue of Ad\'amek's construction of free endofunctor algebras in the $\infty$-categorical setting. We prove that $(\infty, \infty)$-categories with coinductive equivalences form a terminal coalgebra with respect to weak enrichment, and $(\infty, \infty)$-categories with inductive equivalences form an initial algebra with respect to weak enrichment.

==> src/womcats/segal.tex <==
%%!TEX root = ../../article.tex

\subsection{Infinitary Segal spaces}\label{ssec:segal}

In this section, we briefly describe an explicit presentation of (weak) $\omega$-categories via iterated Segal spaces.
We first review the relevant constructions, following \cite[\S1]{lurie:infty2}.

\begin{definition}\label{def:catobj}
    Given an $\infty$-category $\sX$ with finite limits, a \emph{category object} is a functor $\cC:\bDelta^\op\to\sX$ satisfying the \emph{Segal condition}: for every $n\geq0$, the inert morphisms $[0]\to[n]$ and $[1]\to[n]$ induce an equivalence
    \[
        \cC_n \xrightarrow\sim \cC_1\times_{\cC_0}\dots\times_{\cC_0}\cC_1
    \]
    where $\cC_n := \cC([n])$.
    Say that $\cC$ is a \emph{groupoid object} if for every $n\geq0$ and partition $[n] = S\cup T$ with $S\cap T = \{k\}$, the diagram
    $$
    \begin{tikzcd}
        \cC_n \ar[r]\ar[d]\ar[dr, phantom, "\lrcorner" very near start]
        & \cC(T) \ar[d] \\
        \cC(S) \ar[r]
        & \cC(\{k\})
    \end{tikzcd}
    $$
    Denote by $\Cat(\sX)$ and $\Grpd(\sX)$ the full subcategories of $\Fun(\bDelta^\op,\sX)$ on the category objects and groupoid objects, respectively.
\end{definition}
\begin{remark}\label{rem:core}
    By \cite[Proposition 1.1.14]{lurie:infty2}, the inclusion $\Grpd(\sX)\hookrightarrow\Cat(\sX)$ admits a right adjoint $\kappa$.
    When $\sX = \sS$ is the $\infty$-category of spaces, the right adjoint can be constructed as follows.
    Let $i_* : \sS \to \Cat(\sS)$ be given on a space $X$ by setting $(i_*X)_n := X^{\times(n+1)}$.
    For $n\geq0$, let $E^n := i_*\{0,\dots,n\}$, then for any category object $\cC : \bDelta^\op\to\sS$, we obtain a groupoid object $\kappa\cC_\bullet := \Hom(E^\bullet, \cC)$.
    
\end{remark}

\begin{definition}\label{def:absdis}
    For $\sX$ a locally presentable $\infty$-category, let $\sS\subseteq\sX$ denote the unique cocontinuous embedding that preserves the terminal object.
    Say that $\sX$ is an \emph{absolute distributor} if:
    \begin{itemize}
        \item $\sS\subseteq\sX$ is fully faithful and preserves limits.
        \item For all morphisms $X\to S$ in $\sX$ with $S\in\sS$, the pullback functor $\sX_{/S}\to\sX_{/X}$ preserves colimits.
        \item With $\sO$ the full subcategory of $\Fun([1],\sX)$ spanned by the morphisms $X\to S$ with $S\in\sS$, let $\pi:\sO\to\sS$ denote the cartesian fibration given by evaluating at $1\in[1]$, and denote its corresponding functor by $\chi:\sS\to\Cat_\infty^\op$.
            Then, $\chi$ preserves limits.
    \end{itemize}
\end{definition}
\begin{example}\label{ex:basecase}
    $\sS$ itself is an absolute distributor.
\end{example}

\begin{definition}\label{def:css}
    Let $\sX$ be an absolute distributor.
    A \emph{complete Segal space object} in $\sX$ is a category object $\cC : \bDelta^\op\to\sX$ such that
    \begin{itemize}
        \item $\cC_0 \in \sS$ (that is, $\cC$ is a \emph{Segal space}).
        \item $\cC$ is local with respect to the morphism $E^1\to E^0$ of \cref{rem:core}.
    \end{itemize}
    Denote by $\mathbf{CSS}(\sX)$ the full subcategory of $\Cat(\sX)$ spanned by the complete Segal space objects in $\sX$.
\end{definition}
\begin{remark}\label{rem:css}
    If $\sX$ is an absolute distributor, then the inclusion $\sS\subseteq\sX$ admits a right adjoint $\kappa$.
    If $\Seg(\sX)$ denotes the full subcategory of $\Cat(\sX)$ on Segal space objects in $\sX$, then it follows that the inclusion $\Grpd(\sS)\hookrightarrow\Seg(\sS)\subseteq\Seg(\sX)$ admits a right adjoint given by the composite $\Seg(\sX)\xrightarrow{\kappa_*}\Seg(\sS)=\Cat(\sS)\xrightarrow\kappa\Grpd(\sS)$, where the last functor is the right adjoint defined in \cref{rem:core}.

    Now, a Segal space $\cC\in\Seg(\sX)$ is complete if and only if the functor $\kappa\cC\in\Grpd(\sS)$ is essentially constant.
    The equivalence between these definitions is observed in \cite[Proposition 7.16]{haugseng}.
\end{remark}

\begin{theorem}\cite[Corollary 1.3.4]{lurie:infty2}
    If $\sX$ is an absolute distributor, then $\mathbf{CSS}(\sX)$ is an absolute distributor, with $\sS\subseteq\mathbf{CSS}(\sX)$ as the constant functors $\bDelta^\op\to\sS\subseteq\sX$.
\end{theorem}

\begin{theorem}\cite[Theorem 7.18]{haugseng}
    If $\sX$ is an absolute distributor, then with its cartesian monoidal structure, we have an equivalence $\sX\Cat \simeq \mathbf{CSS}(\sX)$, given by sending an $\sX$-category $\cC:\bDelta_S^\op\to\sX^\times$ to the left Kan extension of $\bDelta_S^\op\xrightarrow\cC\sX^\times\to\sX$ (where $\sX^\times\to\sX$ sends $(x_1,\dots,x_n)\mapsto x_1\times\dots\times x_n$) along $\pi:\bDelta^\op_S\to\bDelta^\op$.
\end{theorem}

Combining the above theorems, we obtain a concrete realisation of the $\infty$-category $\Cat_{(\infty, n)}$ for finite $n$ as $n$-fold complete Segal space objects in $\sS$.

\begin{definition}\label{def:Omega}
    Let $\bSigma$ denote the category where:
    \begin{itemize}
        \item The objects are infinite sequences $[\vec k] = (k_0, k_1, k_2, \dots)$ of integers such that there exists some $n\geq0$ such that $k_i > 0$ for all $i < n$, and $k_i = 0$ for all $i \geq n$.
            Call $n$ the \emph{dimension} of $\vec k$, written $n =: \dim[\vec k]$.
        \item The morphisms $\vec\phi : [\vec k]\to[\vec\ell]$ are equivalence classes of infinite sequences of morphisms $\phi_i : [k_i] \to [\ell_i]$ in $\bDelta$, modulo the equivalence where $\vec\phi\sim\vec\phi'$ if there exists some $n\geq0$ such that $\phi_i=\phi'_i$ for all $i < n$, and $\phi_n = \phi'_n = 0$.
            Composition of morphisms is computed levelwise.
    \end{itemize}

    Denote by $\bSigma_n$ the full subcategory of $\bSigma$ spanned by objects of dimension at most $n$.
\end{definition}
\begin{remark}\label{rem:Theta}
    The category $\bSigma_n$ is precisely the quotient category $\bTheta^n$ of $\bDelta^{\times n}$ defined in \cite{simpson:svk}, and $\bSigma \simeq \varcolim_n\bSigma_n$.
\end{remark}
\begin{definition}\label{def:omext}
    For $[\vec k]=(k_0,k_1,k_2)$ an object of $\bSigma$ with $\dim[\vec k] = n$, and $\ell > 0$, denote by $[\vec k,\ell]$ the unique extension of $[\vec k]$ to an object of $\bSigma$ of dimension $n+1$ whose $i$th component is $k_i$ for $i<n$, whose $n$th component is $\ell$, and whose remaining components are zero.
    We can then extend this definition to the case where $\ell=0$ by defining $[\vec k,0] := [\vec k]$.
    This construction defines a fully faithful functor $[\vec k,-] : \bDelta\to\bSigma_{n+1}\subseteq\bSigma$.

    For $[\vec k]$ an object of $\bSigma$, let $\Sigma[\vec k] : \bSigma^\op\to\Set\subseteq\sS$ denote its associated representable functor.
    Given a simplicial space $X:\bDelta^\op\to\sS$, denote by $\Sigma[\vec k,X]$ the left Kan extension of $X$ along the inclusion $[\vec k,-] : \bDelta\hookrightarrow\bSigma$.
\end{definition}
\begin{remark}\label{rem:omext}
    The object $\Sigma[\vec k,X]$ satisfies the following universal property: any $\cC:\bSigma^\op\to\sS$ defines a simplicial space $\cC_{\vec k,\bullet} : \bDelta^\op\to\sS$, and we have a homotopy equivalence
    \[
        \Hom_{\Fun(\bSigma^\op,\sS)}(\Sigma[\vec k,X], \cC) \simeq \Hom_{\Fun(\bDelta^\op,\sS)}(X, \cC_{\vec k,\bullet})
    \]
\end{remark}

\begin{lemma}\label{lem:expl}
    We can identify $\Cat_{(\infty, n)}$ with the full subcategory of $\Fun(\bSigma_n^\op,\sS)$ spanned by those $\cC : \bSigma_n^\op\to\sS$ such that:
    \begin{itemize}
        \item For every $[\vec k]$ with $\dim[\vec k]<n$, and every $\ell>0$, we have a equivalence of spaces
            \[
                \cC_{\vec k,\ell} \xrightarrow\sim \cC_{\vec k,1}\times_{\cC_{\vec k}}\dots\times_{\cC_{\vec k}}\cC_{\vec k,1}
            \]
        \item For every $[\vec k]$ with $\dim[\vec k]<n$, the simplicial space $\cC_{\vec k,\bullet} : \bDelta^\op\to\sS$ is local with respect to the map $E^1\to E^0$.
    \end{itemize}
\end{lemma}
\begin{proof}
    This follows by unwinding the definition of an $n$-fold complete Segal space in $\sS$.
    The first bullet ensures that $\cC_{\vec k,\bullet}$ is a category object for every $[\vec k]$, and thus a Segal space object by the definition of $\bSigma_n$, and the second bullet implies that this Segal space object is complete.
\end{proof}

We now show that the natural extension of this definition to $\bSigma$ recovers $\Cat_{(\infty,\infty)}$:

\begin{theorem}\label{thm:expl}
    We can identify $\Cat_{(\infty,\infty)}$ with the full subcategory of $\Fun(\bSigma^\op,\sS)$ spanned by those $\cC:\bSigma^\op\to\sS$ such that:
    \begin{itemize}
        \item For every $[\vec k]$ and every $\ell > 0$, we have an equivalence of spaces
            \[
                \cC_{\vec k,\ell} \xrightarrow\sim \cC_{\vec k,1}\times_{\cC_{\vec k}}\dots\times_{\cC_{\vec k}}\cC_{\vec k,1}
            \]
        \item For every $[\vec k]$, the simplicial space $\cC_{\vec k,\bullet} : \bDelta^\op\to\sS$ is local with respect to the map $E^1\to E^0$.
    \end{itemize}
    In other words, $\Cat_{(\infty,\infty)}$ is precisely the localisation of $\Fun(\bSigma^\op,\sS)$ at the morphisms
    \[
        \Sigma[\vec k,1]\sqcup_{\Sigma[\vec k]}\dots\sqcup_{\Sigma[\vec k]}\Sigma[\vec k,1] &\to \Sigma[\vec k,\ell], & \Sigma[\vec k,E^1] \to \Sigma[\vec k]
    \]
    for every $[\vec k]$ in $\bSigma$, and every $\ell>0$.
\end{theorem}
\begin{proof}
    Under the identification in \cref{lem:expl}, the inclusion $\Cat_{(\infty,n)}\hookrightarrow\Cat_{(\infty,n+1)}$ is given by identifying an $(\infty, n)$-category with the functor $\bSigma_{n+1}^\op\to\sS$ that is constant at the $(n+1)$st index.
    This is precisely the left Kan extension $i_!:\Fun(\bSigma_n^\op,\sS)\to\Fun(\bSigma_{n+1}^\op,\sS)$ along the inclusion $i:\bSigma_n\subseteq\bSigma_{n+1}$, restricted to higher categories.

    In particular, the right adjoint $\kappa:\Cat_{(\infty, n+1)}\to\Cat_{(\infty,n)}$ is given by restriction along $\bSigma_n\subseteq\bSigma_{n+1}$.
    Therefore,
    \[
        \Cat_{(\infty,\infty)} &:= \varlim\left(\dots\to\Cat_{(\infty,2)}\xrightarrow\kappa\Cat_{(\infty,1)}\xrightarrow\kappa\Cat_{(\infty,0)}\right) \\
            &\subseteq \varlim\left(\dots\to\Fun(\bSigma_2^\op,\sS) \xrightarrow{i^*}\Fun(\bSigma_1^\op,\sS) \xrightarrow{i^*}\Fun(\bSigma_0^\op,\sS)\right) \\
            &\simeq \Fun\left(\varcolim_n\bSigma_n^\op, \sS\right) \\
            &\simeq \Fun\left(\bSigma^\op,\sS\right)
    \]
    identifies $\Cat_{(\infty,\infty)}$ with the full subcategory of $\Fun(\bSigma^\op,\sS)$ spanned by those $\cC:\bSigma^\op\to\sS$ such that $\cC|_{\bSigma_n}$ is an $(\infty, n)$-category in the sense of \cref{lem:expl} for every $n\geq0$.
    The conclusion follows.
\end{proof}
\begin{remark}\label{rem:expl}
    We can then identify $\Cat_{(n, r)}$ with the full subcategory of $\Cat_{(\infty,\infty)}$ spanned by those $\cC:\bSigma^\op\to\sS$ that factor through $\Grpd_n\subseteq\sS$ and are left Kan extensions of their restriction to $\bSigma_r\subseteq\bSigma$.
\end{remark}

\begin{lemma}\label{lem:repcat}
    For $[\vec n]$ in $\bSigma$, the representable object $\Sigma[\vec n]$ is an $(\infty, \infty)$-category.
\end{lemma}
\begin{proof}
    Fix $[\vec k]$ in $\bSigma$, and let $\ell>0$.
    It then follows by the Yoneda lemma that
    \[
        \Sigma[\vec n]_{\vec k,\ell} &= \Hom_\bSigma([\vec k,\ell], [\vec n]) \\
            &\simeq \Hom_\bSigma([\vec k,1]\sqcup_{[\vec k]}\dots\sqcup_{[\vec k]}[\vec k,1], [\vec n]) \\
            &\simeq \Hom_\bSigma([\vec k,1],[\vec n])\times_{\Hom_\bSigma([\vec k],[\vec n])}\dots\times_{\Hom_\bSigma([\vec k],[\vec n])}\Hom_\bSigma([\vec k,1],[\vec n])
    \]
    establishing the Segal condition.
    Regarding completeness, note that a point of $\Sigma[\vec n]_{\vec k}$ is a map $f:[\vec k]\to[\vec n]$ in $\bSigma$, and an arrow $f\to g$ between two such points is a map $h:[\vec k,1]\to[\vec n]$ such that $h|_{\vec k,\{0\}} = f$ and $h|_{\vec k,\{1\}} = g$.
    Such a map only exists if $f_i = g_i$ for every $i < \dim[\vec k]$, and $f_{\dim[\vec k]} \leq g_{\dim[\vec k]}$.

    In particular, if two elements $f, g$ of $\Sigma[\vec n]_{\vec k}$ are connected by arrows $f\to g$ and $g\to f$, then already $f=g$.
    This proves that any map $\Sigma[\vec k,E^1]\to\Sigma[\vec n]$ factors uniquely through the projection $\Sigma[\vec k,E^1]\to\Sigma[\vec k]$, proving completeness of $\Sigma[\vec n]$.
\end{proof}

\begin{corollary}\label{cor:inthom}
    The $\infty$-category $\Cat_{(\infty,\infty)}$ inherits cartesian closed monoidal structure from the ambient category $\Fun(\bSigma^\op,\sS)$; that is, if $\cC,\cD : \bSigma^\op\to\sS$ are $(\infty, \infty)$-categories, then the internal hom $[\cC,\cD] : \bSigma^\op\to\sS$ given by the formula
    \[
        [\cC,\cD]_{\vec k} &:= \Hom_{\Fun(\bSigma^\op,\sS)}(\cC\times\Sigma[\vec k], \cD)
    \]
    is also an $(\infty, \infty)$-category.
\end{corollary}
\begin{proof}
    We have by \cref{prop:inal} that $\Cat_{(\infty,\infty)}$ is presentably symmetric monoidal with respect to its cartesian monoidal structure, which implies that $\Cat_{(\infty,\infty)}$ is a cartesian closed $\infty$-category.
    Let $[-,-]$ denote the internal hom in $\Cat_{(\infty,\infty)}$, then by the Yoneda lemma:
    \[
        [\cC,\cD]_{\vec k} &\simeq \Hom_{\Fun(\bSigma^\op,\sS)}(\Sigma[\vec k],[\cC,\cD]) \\
            &= \Hom_{\Cat_{(\infty,\infty)}}(\Sigma[\vec k],[\cC,\cD]) \tag{\cref{lem:repcat}} \\
            &\simeq \Hom_{\Cat_{(\infty,\infty)}}(\cC\times\Sigma[\vec k],\cD) \\
            &= \Hom_{\Fun(\bSigma^\op,\sS)}(\cC\times\Sigma[\vec k],\cD)
    \]
    as desired.
\end{proof}
\begin{remark}\label{rem:senr}
    This provides an explicit description of the enrichment of $\Cat_{(\infty,\infty)}$ over itself provided by \cite[Corollary 7.4.10]{gepner-haugseng}, producing the large $(\infty, \infty)$-category of $(\infty, \infty)$-categories.
\end{remark}

\FIXME{use the construction of $\Cat_\omega$ to justify proving that $\Cat_\omega$ is a localisation of any presentable fixed point under enrichment, then describe the adjoints explicitly}

\FIXME{}

